Caching for the Future: Scrub Jay Episodic Memory Principles for Agent Memory Systems

LLM agents that persist across sessions accumulate stored memories whose validity varies enormously by content type, yet existing memory architectures treat all memories as equally persistent and systematically contaminate retrieved context with outdated facts. We show that per-memory, type-conditioned temporal decay, a property of western scrub jay episodic memory, can be operationalized as an auto-classified coefficient $\pi_i$ in an external LLM-agent memory store, yielding ScrubJay-MEM: each memory is encoded as a jointly-bound What--Where--When tuple with an estimated perishability $\pi_i$ and utility horizon $\tau_i$, retrieved by query-adaptive scoring, and revised retroactively at $O(1)$ LLM calls per update. We introduce the Temporal Generalization Test (TGT), a benchmark with held-out retention intervals and a Generalization Gap (GenGap) metric. On TGT, ScrubJay-MEM is the only retrieval-based system with substantially positive GenGap ($+0.108$); on MemoryAgentBench EventQA-64k it improves F1 by $+2.66$ over Mem0 and $+3.09$ over Qwen3-Embedding-4B under a llm backbone. A decay ablation collapses GenGap by $5.7\times$, establishing type-conditioned decay as necessary for the result. Gains narrow under stronger backbones and reverse on fact-consolidation tasks, scoping the contribution to temporal reasoning over perishable facts.

==> acl-style-files-master/Section/tgt.tex <==

% =============================================================================
% TGT BENCHMARK SECTION
%   - Main paper: compact subsection introducing the benchmark
%   - Appendix:   full construction details, vocabularies, audit, comparison
%
% Assumes NeurIPS preamble with booktabs, amsmath, amssymb, multirow, graphicx
% =============================================================================


% -----------------------------------------------------------------------------
% MAIN PAPER  —  goes immediately before the §5.3 results subsection
% -----------------------------------------------------------------------------
\subsection{The Temporal Generalization Test}
\label{sec:tgt-benchmark}

To isolate the contribution of explicit temporal modeling, we introduce
the \emph{Temporal Generalization Test} (TGT), a controlled benchmark
that asks whether a memory system generalizes its decay behavior to
retention intervals it has never been calibrated on. TGT is designed
as the computational analog of the avian retention-interval experiments
of \citet{?}, in which western scrub jays were shown to apply learned
decay knowledge to novel, untrained recovery delays---demonstrating a
continuous temporal model rather than memorized behavior at trained
intervals. We argue this generalization property is the right
diagnostic for an episodic memory architecture, and one that no
existing public benchmark for LLM agent memory tests directly.

\paragraph{Design at a glance.}
TGT consists of $20$ independently generated instances, each with $96$
memories drawn from four perishability classes (Ephemeral,
Session-Specific, Durable Preference, Stable Knowledge; $24$ per class)
and $66$ queries issued at five retention intervals. Two of the five
intervals---$I_3$ (medium, 8--12 sessions) and $I_5$ (very long, 40--60
sessions)---are \emph{held out}: no system is permitted to encounter
them during any calibration phase. $I_3$ tests interpolation; $I_5$
tests extrapolation. Ground-truth temporal validity is governed by a
deterministic type$\times$interval schedule (\Cref{tab:tgt-validity}):
ephemeral memories are valid only at the two shortest intervals, stable
knowledge is valid throughout, and the intermediate classes degrade in
between. The full benchmark contains $1{,}320$ query--answer pairs over
$1{,}920$ memories. Construction details, vocabularies, and the quality
audit are deferred to \Cref{app:tgt}.

\begin{table}[t]
  \centering
  \small
  \caption{Ground-truth validity schedule. A memory of type $X$ queried
    at interval $I_k$ is valid iff the corresponding cell is \cmark.
    Held-out intervals are shaded.}
  \label{tab:tgt-validity}
  \begin{tabular}{lccccc}
    \toprule
                       & $I_1$ & $I_2$ & \cellcolor{gray!15}$I_3$ & $I_4$ & \cellcolor{gray!15}$I_5$ \\
                       & immediate & short & \cellcolor{gray!15}medium & long & \cellcolor{gray!15}very long \\
    \midrule
    A: Ephemeral             & \cmark & \cmark & \cellcolor{gray!15}\xmark & \xmark & \cellcolor{gray!15}\xmark \\
    B: Session-Specific      & \cmark & \cmark & \cellcolor{gray!15}\cmark & \xmark & \cellcolor{gray!15}\xmark \\
    C: Durable Preference    & \cmark & \cmark & \cellcolor{gray!15}\cmark & \cmark & \cellcolor{gray!15}\xmark \\
    D: Stable Knowledge      & \cmark & \cmark & \cellcolor{gray!15}\cmark & \cmark & \cellcolor{gray!15}\cmark \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Metric.}
The primary metric is the \emph{Generalization Gap} at the unseen
interpolation interval:
\begin{equation}
  \mathrm{GenGap}(f) \;=\; \mathrm{Acc}(f, I_2) + \mathrm{Acc}(f, I_4) - 2 \cdot \mathrm{Acc}(f, I_3),
  \label{eq:gengap-main}
\end{equation}
where $\mathrm{Acc}(f, I_k)$ is the per-query combined accuracy
(factual correctness $\wedge$ correct staleness judgment, both adjudicated
by an LLM judge from a different model family than the generation
backbone). $\mathrm{GenGap} \approx 0$ indicates that $f$'s behavior at
the unseen $I_3$ interpolates smoothly between the trained $I_2$ and
$I_4$, the signature of a continuous temporal model. Strongly negative
$\mathrm{GenGap}$ indicates the system has memorized behavior at the
trained intervals and fails at the unseen one. We also report the
Temporal Generalization Score $\mathrm{TGS}(f) = \tfrac{1}{5} \sum_k
\mathrm{Acc}(f, I_k)$ and per-interval, per-type, and retrieval-quality
decompositions in the appendix.

